Cross-platform Prediction of Depression Treatment Outcome Using Location Sensory Data on Smartphones

Currently, depression treatment relies on closely monitoring patients response to treatment and adjusting the treatment as needed. Using self-reported or physician-administrated questionnaires to monitor treatment response is, however, burdensome, costly and suffers from recall bias. In this paper, we explore using location sensory data collected passively on smartphones to predict treatment outcome. To address heterogeneous data collection on Android and iOS phones, the two predominant smartphone platforms, we explore using domain adaptation techniques to map their data to a common feature space, and then use the data jointly to train machine learning models. Our results show that this domain adaptation approach can lead to significantly better prediction than that with no domain adaptation. In addition, our results show that using location features and baseline self-reported questionnaire score can lead to F1 score up to 0.67, comparable to that obtained using periodic self-reported questionnaires, indicating that using location data is a promising direction for predicting depression treatment outcome.

==> tables/feature_corr.tex <==
\begin{table}[]
\caption{Pearson’s correlation between location features and self-reported QIDS score for Android and iPhone dataset. \bing{Add a vertical bar separating Android and iPhone results. Change 0.017 to 0.02, change 0.022 to 0.02; so you are consistent in using 2 decimal digits.\soumya{DOne: corrected}  }}

\begin{tabular}{|c|cc|cc|}
\hline
                  & \multicolumn{2}{c||}{\textbf{Android}}          & \multicolumn{2}{c|}{\textbf{{iPhone}}}            \\ \hline
{\textbf{Features }}         & \multicolumn{1}{c|}{\textbf{{r-value}}} & \multicolumn{1}{c||} {\textbf{{p-value}}} & \multicolumn{1}{c|} {\textbf{{r-value}}} & \multicolumn{1}{c|}{\textbf{{p-value}}} \\ \hline

{\textbf{Location variance}} & \multicolumn{1}{c|}{-0.12}   & \multicolumn{1}{c||} {0.05}    & \multicolumn{1}{c|}{- 0.11}  & 0.08    \\ \hline

{\textbf{Time spent moving}} & \multicolumn{1}{c|}{0.06}    &  \multicolumn{1}{c||} {0.56}    & \multicolumn{1}{c|}{0.16}    & 0.01    \\ \hline

{\textbf{Total distance}} & \multicolumn{1}{c|}{-0.09}    & \multicolumn{1}{c||} {0.39}    & \multicolumn{1}{c|}{0.04}    & 0.55    \\ \hline

{\textbf{Average moving speed}} & \multicolumn{1}{c|}{-0.09}    &  \multicolumn{1}{c||}{0.38 }   & \multicolumn{1}{c|}{0.04}    & 0.53    \\ \hline

{\textbf{Unique locations}} & \multicolumn{1}{c|}{0.11}    & \multicolumn{1}{c||} {0.005}   & \multicolumn{1}{c|}{-0.23}    & 0.0003    \\ \hline

{\textbf{Entropy}} & \multicolumn{1}{c|}{0.17}    &  \multicolumn{1}{c||} {0.01}    & \multicolumn{1}{c|}{-0.22}    & 0.001    \\ \hline

{\textbf{Normalized entropy}} & \multicolumn{1}{c|}{0.06}    & \multicolumn{1}{c||}{0.16}   & \multicolumn{1}{c|}{-0.16}    & 0.02    \\ \hline

{\textbf{Time at home}} & \multicolumn{1}{c|}{0.19}    & \multicolumn{1}{c||} {0.04}    & \multicolumn{1}{c|}{0.15}    & 0.02    \\ \hline


\end{tabular}
\end{table}
